DataLens: Scalable Privacy Preserving Training via Gradient Compression and Aggregation

Recent success of deep neural networks (DNNs) hinges on the availability of large-scale dataset; however, training on such dataset often poses privacy risks for sensitive training information. In this paper, we aim to explore the power of generative models and gradient sparsity, and propose a scalable privacy-preserving generative model DATALENS. Comparing with the standard PATE privacy-preserving framework which allows teachers to vote on one-dimensional predictions, voting on the high dimensional gradient vectors is challenging in terms of privacy preservation. As dimension reduction techniques are required, we need to navigate a delicate tradeoff space between (1) the improvement of privacy preservation and (2) the slowdown of SGD convergence. To tackle this, we take advantage of communication efficient learning and propose a novel noise compression and aggregation approach TOPAGG by combining top-k compression for dimension reduction with a corresponding noise injection mechanism. We theoretically prove that the DATALENS framework guarantees differential privacy for its generated data, and provide analysis on its convergence. To demonstrate the practical usage of DATALENS, we conduct extensive experiments on diverse datasets including MNIST, Fashion-MNIST, and high dimensional CelebA, and we show that, DATALENS significantly outperforms other baseline DP generative models. In addition, we adapt the proposed TOPAGG approach, which is one of the key building blocks in DATALENS, to DP SGD training, and show that it is able to achieve higher utility than the state-of-the-art DP SGD approach in most cases. Our code is publicly available at https://github.com/AI-secure/DataLens.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> experiments.tex <==

\begin{table*}[t!]
% \scriptsize
\centering
\caption{\small \textbf{Performance of DP generative models on Image Datasets:} 
Classification accuracy of a model trained on the generated data and tested on real test data under different $\epsilon$ ($\delta=10^{-5}$). %We
%compare \sysname with 
%
%We compare \sysname{} with G-PATE, DP-GAN, PATE-GAN and vanilla DC-GAN. The table presents the ). 
% \bx{MNIST and Fashion-MNIST are 10-class classification problems, while CelebA-Gender and CelebA-Hair are respectively binary  and 3-class datasets.}  
% G-PATE, PATE-GAN, DP-GAN and \sysname{} are both evaluated under two private settings: $\varepsilon=1, \delta=10^{-5}$ and $\varepsilon=10, \delta=10^{-5}$. 
}
%The models that maintains around $75\%$ accuracy of vanilla GAN are marked bold.
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|cccc}
\toprule
\textbf{Dataset} &\textbf{DC-GAN} & &\textbf{DP-GAN} & \textbf{PATE-GAN}  &\textbf{G-PATE} & { \textbf{\name{}} } \\ \midrule
\multirow{2}{*}{\textbf{MNIST}} & \multirow{2}{*}{\shortstack{0.9653 \\  ($\varepsilon=\infty$)}} & $\varepsilon=1$& 0.4036
& 0.4168 & {0.5810} & \textbf{0.7123}  \\ % \cmidrule{3-7}
&   & $\varepsilon=10$ & {0.8011} &  0.6667 &\textbf{0.8092} & {0.8066}  \\ \midrule
\multirow{2}{*}{\textbf{{Fashion-MNIST}}} & \multirow{2}{*}{\shortstack{0.8032 \\ ($\varepsilon=\infty$)}}& $\varepsilon=1$ &0.1053 & 0.4222& {0.5567} &  \textbf{0.6478} \\ % \cmidrule{3-7}
& & $\varepsilon=10$ & 0.6098  & 0.6218 & {0.6934} & \textbf{0.7061}  \\  \midrule
\multirow{2}{*}{\textbf{{CelebA-Gender}}} & \multirow{2}{*}{\shortstack{0.8149 \\  ($\varepsilon=\infty$)}} & $\varepsilon=1$& 0.5330 & 0.6068 & {0.6702} & \textbf{0.7058} \\ % \cmidrule{3-7}
&   & $\varepsilon=10$ & 0.5211 & {0.6535} & {0.6897} & \textbf{0.7287} \\ \midrule
\multirow{2}{*}{\textbf{{CelebA-Hair}}} & \multirow{2}{*}{\shortstack{0.7678 \\ ($\varepsilon=\infty$)}}& $\varepsilon=1$ & 0.3447 & 0.3789& {0.4985} & \textbf{0.6061} \\ % \cmidrule{3-7}
& & $\varepsilon=10$ & 0.3920 & 0.3900 & {0.6217} & \textbf{0.6224}  \\ 
\bottomrule
\end{tabular}%
% }
% \vspace{5pt}
\label{tab:image}
\vspace{-0.5em}
\end{table*}


\begin{table*}[t!]
\centering
\caption{\small \textbf{Performance Comparison of DP generative models on Image Datasets given small privacy budgets.}  ($\delta=10^{-5}$) }
\begin{tabular}{c|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{$\varepsilon$}} & \multicolumn{4}{c|}{\textbf{MNIST}} &  \multicolumn{4}{c}{\textbf{Fashion-MNIST}} \\ 
%\cmidrule(lr){2-3} \cmidrule(lr){4-5}
% \cmidrule{2-5}
 & DP-GAN & PATE-GAN  & G-PATE & \name{} & DP-GAN & PATE-GAN  & G-PATE & \name{} \\
\midrule
0.2 & 0.1104 & 0.2176 & {0.2230} & \textbf{0.2344} & 0.1021  & 0.1605 & 0.1874 & \textbf{0.2226} \\
0.4 & 0.1524 & 0.2399 & {0.2478} & \textbf{0.2919} & 0.1302  & 0.2977 & 0.3020 & \textbf{0.3863} \\
0.6 & 0.1022 & 0.3484 & 0.4184 & \textbf{0.4201} & 0.0998    & 0.3698 & 0.4283 & \textbf{0.4314} \\
0.8 & 0.3732 & 0.3571 & 0.5377 & \textbf{0.6485} & 0.1210    & 0.3659 & 0.5258 & \textbf{0.5534} \\
1.0 & 0.4046 & 0.4168 & 0.5810 & \textbf{0.7123} & 0.1053    & 0.4222 & 0.5567 & \textbf{0.6478} \\
\bottomrule
\end{tabular}
% \vspace{5pt}
\label{tab:lowdp}
\vspace{-0.5em}
\end{table*}

% \vspace{-40pt}


% \vspace{-0.5em}
\section{Experimental Evaluation}
% \vspace{-0.5em}

% \fan{leading paragraph}
In this section, we present the experimental evaluation results of \sysname for generating differentially private data with high utility. We also show the evaluation results of adapting \top to standard DP SGD training.
We first evaluate \sysname for generative models on high-dimensional image data such as
CelebA face datasets to demonstrate the scalability of \top in \sysname. 
We then adapt \top strategy for DP SGD training and observe consistent performance improvements, especially under small privacy budgets.

\subsection{Evaluation of \sysname as DP Generative Models}

In this subsection, we apply \sysname to train a DP generative model and evaluate the utility of the generated data. In particular, we target at high dimensional image datasets to demonstrate the effectiveness of \sysname. Experimental results show that the proposed \sysname can outperform other state-of-the-art DP generative model baselines on different datasets.  

%\vspace{-0.5em}
\subsubsection{Experimental Setup} 
\label{sec:exp-gen-setup}
%\vspace{-0.5em}
% \paragraph{Evaluation Setting.}  
% \textbf{Experimental Setup.}

% \paragraph{Baselines.} 
\hfill\\
We compare the generated data utility of \sysname with three state-of-the-art baselines: DP-GAN~\citep{xie2018differentially}, PATE-GAN~\citep{yoon2018pategan} and, G-PATE~\citep{long2019scalable}. 

\vspace{1mm}
\textbf{Datasets.}\quad
To demonstrate the advantage of \sysname as being able to generate high dimensional differentially private data, we focuse on high dimensional image datasets, including MNIST~\citep{lecun1998mnist}, Fashion-MNIST~\citep{xiao2017fashion}, and CelebA datasets~\citep{liu2015faceattributes}. MNIST and Fashion-MNIST dataset contain grayscale images of $28 \times 28$ dimensions. Both datsets have 60,000 training examples and 10,000 testing examples. The CelebA dataset contains 202,599 color images of celebrity faces. We use the official preprocessed version with face alignment and resize the images to $64 \times 64 \times 3$.

We create two CelebA datasets based on different attributes: CelebA-Gender is a binary classification dataset with gender as the label, while CelebA-Hair uses three hair color attributes (black/ blonde/ brown) as classification labels. The training and testing set is split following the official partition as~\citep{liu2015faceattributes}. 
Since DP-GAN and PATE-GAN did not evaluate their framework on high dimensional image datasets, we run their open-source code and compare with the proposed \sysname framework.


\vspace{1mm}
\textbf{Models.}\quad
Both the teacher discriminator and the student generator of \sysname uses the same architecture as DC-GAN~\citep{radford2015unsupervised}. The latent variables sampled from Gaussian distribution are 50-dimensional for MNIST, 64-dimensional for Fashion-MNIST and 100-dimensional for CelebA datasets. We set top-$k$=200 for MNIST and Fashion-MNIST, and top-$k$=700 for CelebA. 

For baseline models, DP-GAN uses standard WGAN and adds Gaussian noise on the gradients during training to achieve differential privacy. Both PATE-GAN and G-Pate leverage PATE framework to generate differentially private images based on different teacher aggregation strategies. Since DP-GAN and PATE-GAN did not evaluate or report their frameworks on high dimensional image datasets, we run their open-source code of DP-GAN\footnote{Code at \url{https://github.com/illidanlab/dpgan}} and PATE-GAN\footnote{Code at \url{https://bitbucket.org/mvdschaar/mlforhealthlabpub/src/master/alg/pategan/}} and compare with our \sysname framework.  

\textbf{Evaluation Metrics.}\quad
We follow standard evaluation pipelines \citep{long2019scalable, yoon2018pategan}, and evaluate \sysname as well as baselines by training a classifier with the generated data and testing the classifier on real test dataset. We consider the \textit{testing accuracy} on the test set as the indicator for the utility of the synthetic data. We report the accuracy with the optimal parameters we find under corresponding privacy constraints. Ablation studies and discussion on comprehensive hyper-parameter analysis can be found in Section \ref{sec:exp-datalens-result}.
We add the genereated images from \sysname in Appendix Figure \ref{fig:vis} for visualization, and we emphasize that the visual quality of generated images  is orthogonal  to our  goal of generating data with high utility for machine learning. In addition, we can see that the generated images are blurry which is beneficial to protect data privacy.  

\subsubsection{Experimental Results}
\label{sec:exp-gen-results}

\hfill\\

In this section we will evaluate the \sysname on different dataset. We first compare the generated data utility  for \sysname and 3 other state of the art DP generative model baselines.
We then explore the impacts of different hyper-parameters and the performance of \sysname under limited privacy budgets, which is a more challenging while important scenario. We show that the proposed \sysname not only outperforms all baselines, but also demonstrates its additional  advantages especially when the privacy budget is small.



\indent {\textbf{Data Utility Evaluation.}}\quad
We first compare \sysname with three baselines
under two privacy budget settings $\varepsilon=1, \delta=10^{-5}$ and  $\varepsilon=10, \delta=10^{-5}$ for four high dimensional image datasets,
following the standard evaluation pipeline. 

From Table \ref{tab:image}, we can see that \sysname shows substantially higher performances than other baseline methods especially when $\varepsilon=1$. In particular, the performance improvement on MNIST under $\varepsilon=1$ is more than $13\%$. Even for CelebA-Hair dataset whose dimensionality is 16 times larger than MNIST, \sysname achieves $10\%$ higher performance improvement than the state of the art, which demonstrates its advantages on high dimensional data than other baseline DP generative models. 
% For $\varepsilon=10$, \sysname also shows better performances than baseline methods on most datasets. On MNIST, \sysname is only $0.0026$ lower than the state of the art, which confirms that our algorithm is a state-of-the-art algorithm under various privacy constraints.   

% \vspace{-0.5em}
\textbf{Ablation studies on small privacy budgets.}
To further demonstrate that \sysname is able to generate high-utility images under small privacy budgets (o.e. higher private protection guarantees), we conduct ablation studies on MNIST and Fashion-MNIST under $\varepsilon \le 1$. 


The experimental results are shown in Table \ref{tab:lowdp}. We find that \sysname shows the best results compared with the baselines given such tight privacy constraints.  With increasing privacy budgets, different DP models gradually converge and the accuracy stably increases. We note that \sysname converges the fastest and achieves more than $20\%$ accuracy even under smallest privacy buddget $\varepsilon=0.2$ for both MNIST and Fashion-MNIST datasets, while baseline models barely converge and the accuracy is similar to the performance of random guess. The observed experimental results also support our theoretical analysis that the proposed \top algorithm can introduce a smaller bias and provide high-utility gradient information for the student generator to converge, confirming that our method is particularly effective under limited privacy budgets.
% the following experiments on the DP-SGD training also confirm this phenomenon.


% \vspace{-0.5em}
\textbf{Ablation studies on hyper-parameters.}\quad
\label{sec:exp-datalens-result}
As we can see, \sysname contains several key hyper-parameters: the number of the teacher models, the top-$k$, and the threshold $\beta$, the standard deviation $\sigma$ of injected Gaussian noise, and the gradient clipping constant $c$. We evaluate a set of hyper-parameters as shown in Table \ref{tab:projection_teachers_1} and Table~\ref{tab:projection_teachers_2}. For other parameters, we searched for the optimal combinations: for MNIST and Fashion-MNIST datasets, we set $\sigma=5000$ when $\varepsilon=1$ and $\sigma=900$ when $\varepsilon=10$; for CelebA datasets of higher dimensionality, we set $\sigma=9000$ when $\varepsilon=1$ and $\sigma=700$ when $\varepsilon=10$. We set the gradient clipping constant $c=10^{-5}$ in all experiments. We also follow the default DC-GAN model configuration\footnote{Details can be found at \url{https://github.com/carpedm20/DCGAN-tensorflow}.} and set the batch size the same as disjoint data partition size.

From Table \ref{tab:projection_teachers_1} and Table~\ref{tab:projection_teachers_2}, we observe that training more teacher discriminators will give us better performance in general, as it can save more privacy budgets. However, with more teacher discriminators, each discriminator will have the access to a smaller amount of training data, thus leading to a slightly worse performance. We observe this trade-off on the CelebA-Gender dataset, where the optimal number of teachers is $6000$. Choosing a proper top-$k$ and $\beta$ is bit tricky: as stated in the discussion of Section \ref{sec:discussion}, if top-$k$ is too small, the model converges slower and is likely to converge to a bad solution. However, if top-$k$ is too large, we will introduce a larger differential privacy noise and the model can soon reach the privacy budget given the high sensitivity. In this paper, we search for the best top-$k$ via grid search. Another observation is that we usually need to set a high threshold $\beta$ to smooth out the noisy gradient entries from the differential privacy noise. However, if the threshold is too high, it is likely to ignore the top-$k$ voted gradients information. This tradeoff leads us to choose a threshold $\beta$ between $\frac{\sigma}{2N}$ and $\frac{\sigma}{N}$.


\begin{table}[t]
% \scriptsize
\centering
% \vspace{-15pt}
\caption{\small \textbf{Impact of different hyper-parameters: the number of Teachers, top-$k$ and threshold $\beta$ for MNIST and Fashion-MNIST datasets under $\epsilon=1$.} We search for the optimal parameter combinations and report the best accuracy by controlling the parameter in each cell.
% We use 4000 teachers and the best $\beta$ to evaluate top-$k$; top-$k$=200 for \# teachers; and top-$k$=200 with 4000 teachers for $\beta$.
% We performed comprehensive studies on the number of teachers and the the projection dimensions on MNIST with $\varepsilon=1$ and $\delta=10^{-5}$. The model has the best performance with 4000 teacher models and TopK equals to 200.
} %.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\toprule
\multirow{2}{*}{}  & \multicolumn{3}{c|}{\textbf{Top-$k$}} & \multicolumn{3}{c}{\textbf{\# of Teachers}} \\ 
&  100 &  {200} & 300  & 2000  & 3000  & {4000}  \\ \midrule
\textbf{MNIST} & 0.5889  & \textbf{0.7123}  & 0.6753  & 0.5841 & 0.7061  & \textbf{0.7123}   \\ 
\textbf{Fashion} & 0.5738  & \textbf{0.6478} & 0.6088 & 0.5608 & 0.5952 & \textbf{0.6478}  \\ \bottomrule
\toprule
$\beta$ &  0 & 0.1 & \multicolumn{1}{c}{0.3} & 0.5 & 0.7 & 0.9  \\ \midrule
\textbf{MNIST} & 0.6361 & 0.6450  & \multicolumn{1}{c}{0.6890} & 0.6921 & \textbf{0.7123} & 0.6956   \\ 
\textbf{Fashion} & 0.5859 & 0.6103 & \multicolumn{1}{c}{0.6060}  & 0.6122 & 0.6213 & \textbf{0.6478}  \\ 
\bottomrule
\end{tabular}%
}
\label{tab:projection_teachers_1}
\vspace{-0.8em}
\end{table}

\begin{table}[t]
% \scriptsize
\centering
% \vspace{-15pt}
\caption{\small \textbf{Impact of Teachers \#, top-$k$ and threshold $\beta$ for CelebA datasets under $\epsilon=1$.} We search for the optimal parameter combinations and report the best accuracy by controlling the parameter in each cell.
% We use 4000 teachers and the best $\beta$ to evaluate top-$k$; top-$k$=200 for \# teachers; and top-$k$=200 with 4000 teachers for $\beta$.
% We performed comprehensive studies on the number of teachers and the the projection dimensions on MNIST with $\varepsilon=1$ and $\delta=10^{-5}$. The model has the best performance with 4000 teacher models and TopK equals to 200.
} %.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\toprule
\multirow{2}{*}{}  & \multicolumn{3}{c|}{\textbf{Top-$k$}} & \multicolumn{3}{c}{\textbf{\# of Teachers}} \\ 
&  500 & {700}  & 900  &  4000  & 6000  & 8000  \\ \midrule
\textbf{CelebA-Gender} & 0.6922 & \textbf{0.7058}  &  0.6811  &  0.6378  &  \textbf{0.7058}  & 0.6936   \\ 
\textbf{CelebA-Hair} & 0.5792   &  \textbf{0.6061} &  0.5769  & 0.5669 &  0.5835 &  \textbf{0.6061} \\ \bottomrule
\toprule
$\beta$ &  0.5  & 0.6 & \multicolumn{1}{c}{0.7}  & 0.8 & 0.85 & 0.9  \\ \midrule
\textbf{CelebA-Gender} & 0.6440   &  0.6789 & \multicolumn{1}{c}{0.6922} & 0.6861 &  \textbf{0.7058} & 0.6381 \\ 
\textbf{CelebA-Hair} &  0.4957 &  0.5669 & \multicolumn{1}{c}{0.5612}  & {0.6022}  & 0.5835 & \textbf{0.6061} \\ 
\bottomrule
\end{tabular}%
}
\label{tab:projection_teachers_2}
\vspace{-0.8em}
\end{table}



\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/dpsgd-mnist.pdf}
        \caption{MNIST}
    \end{subfigure}
    \begin{subfigure}[t]{.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/dpsgd-cifar-small.pdf}
        \caption{CIFAR-10 (under small $\varepsilon$)}
    \end{subfigure}
        \begin{subfigure}[t]{.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/dpsgd-cifar-large.pdf}
        \caption{CIFAR-10 (under full range of $\varepsilon$)}
    \end{subfigure}
    % \includegraphics[width=.33\linewidth]{figures/dpsgd-mnist.pdf}
    % \includegraphics[width=.33\linewidth]{figures/dpsgd-cifar-small2.pdf}
    % \includegraphics[width=.33\linewidth]{figures/dpsgd-cifar-large2.pdf}
    \caption{\small The performance of \sysname applied to SGD training on two datasets: (a) MNIST and (b-c) CIFAR-10.
    We run \sysname with a range of $k\in\{0.7,0.8,1.0\}$ and compare its performance with two baselines GM-DP and DPDL on a wide range of privacy budget $\eps$. % \fan{TODO for Boxin for (b-c): 1) remove the figure title in the plot; 2) use marker=`.'}
}
    \label{fig:dpsgd}
\end{figure*}



\subsection{Evaluation of \top for DP SGD Training}
\label{sec:exp-sgd-setup}

In this section, we demonstrate the universality of the proposed DP gradient compression and aggregation algorithm \top in \sysname, and in particular, the feasibility of applying it to DP SGD training by 
evaluating its performance on two standard image classification tasks for evaluating DP SGD mechanisms.
% In this section, we
% evaluate the performance of \sysname when applied to SGD training to demonstrate the universality of our framework. 
We first describe the experimental setup.
Then we provide extensive evaluation results on a wide range of privacy budgets. 
Overall, the results show that the \top enabled DP SGD training achieves similar or even better performance on model utility compared with the state-of-the-art Gaussian DP mechanism based on the Moment Account~\citep{mcmahan2019tfprivacy} (we will call it \gmdp in the rest of the paper). We also show that \top would bring additional advantages  under limited privacy budgets, where the utility gap between DP and vanilla model is large for traiditional DP approaches.

\subsubsection{Experimental Setup}\hfill\\
We evalute \top for DP SGD training on two datasets, and compare its performance with two baseline frameworks, including the differentially private deep learning (DPDL)~\citep{Abadi2016DeepLW} and \gmdp~\citep{mcmahan2019tfprivacy}.

\textbf{Datasets.}\quad
We experiment with two datasets commonly used in DP SGD research: MNIST~\citep{lecun1998mnist} and CIFAR-10~\citep{cifar10}.
Both datasets are standard image classification datasets. 
The description of MNIST is provided in Section~\ref{sec:exp-gen-setup}. Similarly, we use 60,000 instances for training and 10,000 for testing.
CIFAR-10 is consisted of 60,000 32$\times$32 colored images of 10 classes. Among all, 50,000 instances are used in training while 10,000 are used in testing.

\textbf{Models.}\quad
For MNIST, we adopt a simple convolutional neural network following the default model architecture 
% The model architecture is the same as the following the 
given in the example in the open source Opacus library\footnote{Code at \url{https://github.com/pytorch/opacus/blob/master/examples/mnist.py}}.
% The structure of the network is borrowed from the example given in the Opacus library
The network is consisted of 
two convolutional layers each followed by a max pooling layer, as well as two fully connected layers on the top.
% \boxin{We follow the default model architectures, or what is the hyper-parameters of models?}
% a convolutional layer of channel size 16, kernel size 8, stride size 2, padding size 3, 
% a max pooling layer of stride size 2,
% another convolutional layer of channel size 32, kernel size 4, stride size 2, padding size 1, 
% as well as another max pooling layer also of stride size 2.
% Two fully connected layers each with 32 output neurons and 10 neurons are placed on the top.
% \fan{model for CIFAR-10}

For CIFAR-10, we follow the setting of DPDL, where classifiers are first pretrained on public datasets, then freeze the parameters of feature extractor and  finetune on the fully connected layers. In our paper, we use ResNet-18 \citep{he2016deep} as the architecture of the classifier and load the model parameters pretrained on ImageNet\footnote{Publicly available at \url{https://pytorch.org/docs/stable/torchvision/models.html}}. We replace the fully connected layer with a randomly initialized linear head that takes features of $512$-dimension extracted from ResNet feature extractor as input and outputs $10$-dimensional prediction logits. During training, we freeze the parameters of ResNet feature extractor including the parameters of Batch Normalization layers to ensure that the feature extractor will not leak any privacy-sensitive data information. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% baseline ver 2: TF-Privacy
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We compare the performance of \top with two state of the art DP SGD mechanisms: 
\gmdp~\citep{mcmahan2019tfprivacy} and DPDL~\citep{Abadi2016DeepLW}.
% PyTorch Opacus~\citep{opacus2020} and the results in Abadi \textit{et al.}~\citep{abadi2016deep}.
In particular, we build upon Opacus~\citep{opacus2020}, a PyTorch implementation of \gmdp that implements the DP SGD training scheme and privacy accountant method in~\citep{mcmahan2019tfprivacy}, which enables  convenient control of randomness in the framework.
Our implementation of \top for DP SGD training is also  built upon the Opacus library.
For DPDL which is the first work that proposed and evaluated the DP SGD training scheme, we directly compare with the  results reported in Section 5.2 and Section 5.3 of the paper for fairness, which present the best model utility performance.
% For ease of reference, we will address the two baselines as \textit{TF-Privacy} and \textit{DPDL} in later mentions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% baseline ver 1: Opacus
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We compare the performance of \sysname with two baselines: 
% PyTorch Opacus~\citep{opacus2020} and the results in Abadi \textit{et al.}~\citep{abadi2016deep}.
% PyTorch Opacus is an open-source differential privacy framework which implements the SGD training scheme and privacy accountant method in~\citep{mcmahan2019tfprivacy}.
% Abadi \textit{et al.} is the first work that proposed and evaluated the DP SGD training scheme.
% For ease of reference, we will use the names \textit{Opacus} and \textit{DPDL} to address the two baselines in later reference.
% % We use two open-source differential privacy frameworks, PyTorch Opacus~\citep{opacus2020} and TensorFlow Privacy~\citep{mcmahan2019tfprivacy}, to train the baseline models.
% % Both frameworks are implemented based on the SGD training scheme proposed in~\citep{abadi2016deep}.
% Particularly, our implementation of \sysname for SGD training is further built upon the Opacus library.

% For all the models, we train the network to minimize the cross-entropy loss on the intended classification task. 

\vspace{1mm}
\textbf{Evaluation Metrics.}\quad
We evaluate the model utility, which is calculated as the \textit{classification accuracy} of the trained models,  as the evaluation metric for assessing the effectiveness of our algorithm \top. 
For each dataset, each privacy budget $\eps$, and each \texttt{NormTopK} parameter $k$, we perform an extensive grid search for the combination of hyper-parameters (including gradient clipping norm $C$, noise scale $\sigma$, batch size $B$, and learning rate $lr$) for all methods for fair comparison.
We then use the best hyper-parameters to start 10 runs with different random seeds for noise generation and report the averaged results for each method. 
For models trained under baseline frameworks, we follow the same parameter search protocol and parameter grid to obtain the 
the reported results. 
\vspace{-0.3em}
\subsubsection{Experimental Results}
\input{tables/tab_sgd}
\label{sec:exp-sgd-results}
\hfill\\
We compare \top (with $k\in\{0.7, 0.8, 1.0\}$) with two baselines (\gmdp and DPDL) on DP SGD training under a wide variety of privacy constraints, as shown in Figure~\ref{fig:dpsgd}. 
For clarity of presentation, we leave the complete set of results in Table~\ref{tab:dpsgd}.
% the observations and conclusions are similar.
For MNIST, we mainly evaluate small privacy budgets ($\eps\leq 1.0$), since the performance gap of private and non-private models on MNIST is negligible for large $\varepsilon$.
For CIFAR-10, specifically, we examine the regions of both small $\eps$ and large $\eps$ respectively in a more comprehensive manner.

We first note that \gmdp is a special case of our \top when $k=1.0$. In this case, the complete gradient is preserved after the Top-K step, and therefore the performance of \top is equivalent to \gmdp.
Still, we provide both results as a sanity check in Figure \ref{fig:dpsgd}. We observe that
the results of \top ($k=1.0$) and \gmdp are indeed close in almost all scenarios regardless the randomness of the algorithm (the green and red lines are generally overlapped).

In Figure \ref{fig:dpsgd} (a) for MNIST, different curves are intertwined, indicating that choosing different $k$ values can only influence the model performance by a little margin.
Therefore, it does not hurt to adopt \top with different $k$. The main reason is that, on MNIST, the model utility gap before and after adding DP noise is small which does not provide space for different gradient compression ratios to improve the performance.

Moreover, for CIFAR-10, we observe consistent performance improvements under limited privacy budget $\epsilon$ in Figure \ref{fig:dpsgd} (b), which is also aligned with our observation in \top for generative models, where our methods demonstrate a large margin over baselines under limited privacy budgets. Specifically, In Table \ref{tab:dpsgd} (b) under $\varepsilon=0.025$, we observe that \top  with $k=0.8$ can achieve the model accuracy of $45.87\%$, which is more than $4\%$ higher than the baseline. This again verifies our theoretical analysis that \top can help save the privacy budget consumption by compressing the gradient, and therefore substantially help the model convergence and improve the utility of the model. 

With larger privacy budgets, Figure \ref{fig:dpsgd} (c) shows that \top with very small $k$ tends to have worse performance. It indicates that given small $k$, the bias introduced by top-$k$ compression outweighs the bias introduced by low differential privacy noise. Without DP noise ($\varepsilon=\infty$), we observe that \top with $k < 1$ has slightly worse  performance than the \gmdp baseline, which is because without DP noise there is no longer the benefits of lower DP noise brought by top-$k$, while the bias introduced by gradient compression starts to hurt the performance by a small margin.

We further point out that DPDL has the worst performance among all as shown in Figure~\ref{fig:dpsgd}. This phenomenon is well understood given that the privacy analysis is looser in Abadi et al.~\citep{Abadi2016DeepLW} compared with the privacy analysis based on R\'enyi Differential Privacy~\citep{mironov2019r} adopted in both our \top and \gmdp here.

In addition, we empirically analyze the hyper-parameters and the impact of gradient compression and noise injection in \top on MNIST.  We omit the detailed results in Appendix~\ref{sec:appen-top}. We observe that the bias induced by the DP noise is indeed larger than the gradient compression, which confirms our theoretically analysis of the convergence for \top. 


\vspace{1mm}

% \vspace{-12pt}



% \begin{table}[t]\small 
% \centering
% \vspace{-10pt}
% \caption{\textbf{Performance on Image Datasets.} We compare \sysname{} with G-PATE, DP-GAN and vanilla DC-GAN. The table presents the classification accuracy of a model trained on the generated data and tested on real data. 
% % \bx{MNIST and Fashion-MNIST are 10-class classification problems, while CelebA-Gender and CelebA-Hair are respectively binary  and 3-class datasets.}  
% G-PATE, DP-GAN and \sysname{} are both evaluated under two private settings: $\varepsilon=1, \delta=10^{-5}$ and $\varepsilon=10, \delta=10^{-5}$.}
% \begin{tabular}{l||c||c|c|c||c|c|c}
% \toprule
% \multirow{2}{*}{Dataset} & \textbf{DC-GAN} & \textbf{DP-GAN} & \textbf{G-PATE} &\textbf{\name{}}   & \textbf{DP-GAN} & \textbf{G-PATE} &\textbf{\name{}}  \\ \cmidrule{2-8}
%  &  $\varepsilon=\infty$ & \multicolumn{3}{c||}{$\varepsilon=1$} & \multicolumn{3}{c}{$\varepsilon=10$}    \\ \midrule
% {\textbf{MNIST}} & {{0.9653 }} & 0.4036  & {0.5810} & \textbf{0.7123} & 0.8011  &\textbf{0.8092} & 0.8066  \\ \midrule
% {\textbf{{Fashion-MNIST}}} & 0.8032  &0.1053 & {0.5567} &  \textbf{0.6213} & 0.6098  & {0.6934} & \textbf{0.7061}  \\ 
% \midrule
% \textbf{{CelebA-Gender}} & 0.8149 & 0.5330 & {0.6702} & \textbf{0.7058} & 0.5211  & {0.6897} & \textbf{0.7287} \\ \midrule
% \textbf{{CelebA-Hair}} & 0.7678  & 0.3447 & {0.4985} & \textbf{0.5835}  & 0.3920  & \textbf{0.6217} & {0.6022}  \\ 
% \bottomrule
% \end{tabular}
% % \vspace{5pt}
% \label{tab:image}
% \vspace{-2mm}
% \end{table}





==> framework_overview.tex <==
Figure~\ref{fig:overview} presents an overview for the structure of \sysname. The model introduces a novel algorithm for high dimensional differentially private (DP) gradient compression and aggregation, combined with the PATE framework~\citep{papernot2018scalable}. The framework consists of an ensemble of teacher discriminators and a student generator. The teacher discriminators have access to randomly partitioned  non-overlapping sensitive training data. In each training iteration, each teacher model produces a gradient vector to guide the student generator to update its synthetic record. These gradient vectors are aggregated using a DP gradient aggregation algorithm before being sent to the student generator.

\begin{figure}
% \vspace{-0.5em}
\includegraphics[width=\linewidth]{figures/DataLens.pdf}
% \vspace{-1.5em}
\caption{\small \textbf{Overview of \sysname.} \sysname consists of an ensemble of teacher discriminators and a student generator. \sysname provides a novel algorithm for \emph{high dimensional DP gradient compression and aggregation}. The algorithm consists of two parts: (1) top-$k$ and
sign gradient compression that selects the top $k$ gradient directions, and (2) DP gradient aggregation for high-dimensional gradient aggregation.}
\label{fig:overview}
% \vspace{-6mm}
\end{figure}


The DP gradient aggregation algorithm is crucial for the privacy and utility of the generator. Yet, it is challenging for the algorithm to both preserve high utility and achieve a strong privacy guarantee. On the one hand, to achieve high utility, the algorithm need to preserve the true gradient directions of the teacher models. On the other hand, privacy composition over a high dimensional gradient vector often consumes high privacy budget, resulting in a weaker privacy guarantee. 

To address this problem, prior work uses random projection to project the gradient vector onto lower dimensions~\citep{long2019scalable}. However, this approach introduces excessive noise to the gradient directions and greatly limits the utility of the model. 

In \sysname, we propose a novel algorithm for high dimensional DP gradient compression and aggregation. Our main insight hinges on gradient vectors
as indicated in recent 
work about distributed learning~\citep{NIPS2017_6768, NIPS2018_7837}: 
we can apply aggressive lossy
compression on the 
gradient vectors without
slowing down SGD convergence.
In this paper, we identify
a specific lossy compression scheme under which we can 
leverage more efficient DP mechanism; thus
increase the utility significantly.

%First, the direction of a gradient vector plays a much more important role than its magnitude. Second, the direction of a gradient vector is mostly determined by its entries with the highest absolute values~\citep{xxxx}. 

Our proposed gradient compression algorithm takes the top-$k$ entries in a gradient vector and compresses them via stochastic sign gradient quantization~\citep{jin2020stochastic}. This step significantly reduces the dimensionality of a gradient vector while preserving the most valuable gradient direction information. After the compression, we perform DP gradient aggregation over the sign gradient vectors with a corresponding noise injection mechanism. Since the gradient vectors have been compressed, the aggregation algorithm has a much lower sensitivity, which leads to a tighter privacy bound. 


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> privacy_background.tex <==
We first recall the definitions for differential privacy, R\'enyi differential privacy, and related theorems. 
\bo{Yunhui, we may want to motivate the section for privacy analysis more and emphasize our novelties as well}
% \vspace{-0.5em}
\paragraph{Differential Privacy.}
$(\varepsilon,\delta)$-differential privacy ($(\varepsilon,\delta)$-DP) is a gold standard of privacy proposed by Dwork et al.~\citep{dwork2008differential}. It bounds the change in output distribution caused by a small input perturbation of a randomized algorithm. The following definition formally describes this privacy guarantee.
\begin{definition}[$(\varepsilon, \delta)$-Differential Privacy~\citep{dwork2008differential}]
\label{def:dp}
A randomized algorithm $\mathcal{M}$ with domain $\mathbb{N}^{|\mathcal{X}|}$ is $(\varepsilon,\delta)$-differentially private if for all $\mathcal{S} \subseteq \Range{\mathcal{M}}$ 
and for any neighboring datasets $D$ and $D'$:
\begin{equation*}
    \Pr[\mathcal{M}(D) \in \mathcal{S}] \leq \exp(\varepsilon)\Pr[\mathcal{M(D')\in \mathcal{S}}] + \delta.
\end{equation*}
\end{definition}

Differential privacy is immune to post-processing. Formally, the composition of a data-independent mapping $g$ with an $(\varepsilon, \delta)$-DP mechanism $\mathcal{M}$ is also $(\varepsilon, \delta)$-DP~\citep{dwork2014algorithmic}. 

% \vspace{-0.5em}
\paragraph{R\'enyi Differential Privacy.} 
Defined below, R\'enyi differential privacy (RDP) relaxes DP by measuring the output distribution shift using R\'enyi divergence. 
\begin{definition}[$(\lambda, \alpha)$-RDP~\citep{mironov2017renyi}]
\label{def:rdp}
A randomized mechanism $\mathcal{M}$ is said to guarantee $(\lambda, \alpha)$-RDP with $\lambda > 1$ if for any neighboring datasets $D$ and $D'$,
\begin{small}
\begin{equation*}
    D_{\lambda}\left(\mathcal{M}(D) \| \mathcal{M}\left(D^{\prime}\right)\right) = 
    \frac{1}{\lambda-1} \log \mathbb{E}_{x \sim \mathcal{M}(D)}\left[\left(\frac{\mathbf{P} \mathbf{r}[\mathcal{M}(D)=x]}{\mathbf{P r}\left[\mathcal{M}\left(D^{\prime}\right)=x\right]}\right)^{\lambda-1}\right] \leq \alpha.
\end{equation*}
\end{small}
\end{definition}

For any given probability $\delta>0$, $(\lambda, \alpha)$-RDP implies $(\varepsilon_\delta, \delta)$-differential privacy with $\varepsilon_\delta$ bounded by the following theorem.
\begin{theorem}[From RDP to DP~\citep{mironov2017renyi}]
\label{theorem:rdp-dp}
If a mechanism $\mathcal{M}$ guarantees $(\lambda, \alpha)$-RDP, then $\mathcal{M}$ guarantees $(\alpha + \frac{\log 1/\delta}{\lambda-1}, \delta)$-differential privacy for any $\delta \in (0,1)$.
\end{theorem}

Suppose $f$ is a real-valued function, and the Gaussian mechanism is defined as follows: 
\begin{small}
\begin{equation*}
    \mathbf{G}_{\sigma} f(D)=f(D)+\mathcal{N}\left(0, \sigma^{2}\right),
\end{equation*}
\end{small}where $N\left(0, \sigma^{2}\right)$ is normally distributed random variable. The Gaussian mechanism provides the following RDP guarantee:
\begin{theorem}[RDP Guarantee for Gaussian Mechanism~\citep{mironov2017renyi}]
\label{theorem:rdp-gaussian}
If $f$ has $\ell_2$-sensitivity $s$, then the Gaussian mechanism $\mathbf{G}_{\sigma}f$ satisfies $\left(\lambda, s^2 \lambda /\left(2 \sigma^{2}\right)\right)$-RDP.
\end{theorem}

RDP is also preserved by post-processing. That is, any composition of a data-independent mapping $g$ with an $(\lambda, \alpha)$-RDP mechanism $\mathcal{M}$ is also $(\lambda, \alpha)$-RDP~\citep{mironov2017renyi}.

% \vspace{-0.5em}
\paragraph{Data-Dependent RDP.} The parameters $\varepsilon$ in Definition~\ref{def:dp} and $\alpha$ in Definition~\ref{def:rdp} are called \emph{the privacy budget} of a randomized mechanism. When $\varepsilon$ and $\alpha$ are dependent of the input dataset $D$, the privacy bound is data-dependent. Papernot et al.~\citep{papernot2018scalable} proposed a data-dependent RDP bound for randomized algorithms satisfying RDP guarantees. 

\begin{theorem}[Data-Dependent RDP Bound~\citep{papernot2018scalable}]
\label{theorem:rdp-dependent}
Let $\mathcal{M}$ be a randomized algorithm with $(\mu_1,\alpha_1)-$RDP and $(\mu_2,\alpha_2)-$RDP guarantees and suppose that there exists a likely outcome $i^{*}$ given
a dataset $D$ and a bound $\Tilde{q}\leq 1$ such that $\tilde{q} \geq \operatorname{Pr}\left[\mathcal{M}(D) \neq i^{*}\right]$. Additionally, suppose that $\lambda \leq \mu_{1}$ and $\tilde{q} \leq e^{\left(\mu_{2}-1\right) \alpha_{2}} /\left(\frac{\mu_{1}}{\mu_{1}-1} \cdot \frac{\mu_{2}}{\mu_{2}-1}\right)^{\mu_{2}}$. Then, for any neighboring dataset $D'$ of $D$, we have:
\begin{small}
\begin{equation*}
D_{\lambda}\left(\mathcal{M}(D) \| \mathcal{M}\left(D^{\prime}\right)\right) \leq \frac{1}{\lambda-1} \log \left((1-\tilde{q}) \cdot \boldsymbol{A}\left(\tilde{q}, \mu_{2}, \alpha_{2}\right)^{\lambda-1}+\tilde{q} \cdot \boldsymbol{B}\left(\tilde{q}, \mu_{1}, \alpha_{1}\right)^{\lambda-1}\right),
\end{equation*}
\end{small}
where $\boldsymbol{A}\left(\tilde{q}, \mu_{2}, \alpha_{2}\right) \triangleq(1-\tilde{q}) /\left(1-\left(\tilde{q} e^{\alpha_{2}}\right)^{\frac{\mu_{2}-1}{\mu_{2}}}\right)$ and $\boldsymbol{B}\left(\tilde{q}, \mu_{1}, \alpha_{1}\right) \triangleq e^{\alpha_{1}} / \tilde{q}^{\frac{1}{\mu_{1}-1}}$.
\end{theorem}
The parameters $\mu_1$ and $\mu_2$ are optimized to get a data-dependent RDP guarantee for any order $\lambda$. 

This data-dependent privacy bound improves on the data-independent one as long the distribution of the algorithm's output on that input has a strong peak (i.e.$  q \ll 1$)~\citep{papernot2018scalable}. 

==> tables/append_dpsgd.tex <==
\subsection{Related Work for DP SGD Training} 
% Differential privacy~\citep{dwork2008differential}, 
DPDL~\citep{Abadi2016DeepLW} is the first work that applies the notion of Differential Privacy to the SGD training to prevent deep neural models from exposing private information of training data. DPDL also proposes to compute the privacy cost of the training by moments accountant, which proves to be a tighter bound than the strong composition theorem. \citet{mcmahan2019tfprivacy} adopts the notion of R\'enyi differential privacy, which extends and generalizes the moment accountant to multi-vector queries. Thus, the R\'enyi differential privacy analysis enables the framework to provide privacy for heterogeneous sets of vectors and is widely adopted by current open-source DP library (Tensorflow Privacy and Pytorch Opacus) implementation.
However, the high-dimensional data issue is still present in these algorithms given the fact that the privacy budget can be consumed quickly when aggregating these gradients in a differentially private manner.


==> tables/fig_dp_bound.tex <==
\begin{figure*}[th]
    \centering
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mnist-eps.pdf}
        \caption{MNIST}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fmnist-eps.pdf}
        \caption{Fashion-MNIST}
    \end{subfigure}
        \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/hair-eps.pdf}
        \caption{CelebA-Hair}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gender-eps.pdf}
        \caption{CelebA-Gender}
    \end{subfigure}
    % \includegraphics[width=.33\linewidth]{figures/dpsgd-mnist.pdf}
    % \includegraphics[width=.33\linewidth]{figures/dpsgd-cifar-small2.pdf}
    % \includegraphics[width=.33\linewidth]{figures/dpsgd-cifar-large2.pdf}
    \caption{Ablation studies on the data dependent bound v.s. data independent bound. The data independent bound always yields tighter privacy bound than the data dependent analysis, given the high dimensionality of the gradients.
}
    \label{fig:dept_bound}
\end{figure*}

==> tables/tab_hyperpara_celeba.tex <==
\begin{subtable}[h]{\columnwidth}
% \label{tab:projection_teachers_2}
% \caption{Evaluation on CelebA-Hair and CelebA-Gender datasets}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\toprule
\multirow{2}{*}{}  & \multicolumn{3}{c|}{\textbf{Top-$k$}} & \multicolumn{3}{c}{\textbf{\# of Teachers}} \\ 
&  500 & {700}  & 900  &  4000  & 6000  & 8000  \\ \midrule
\textbf{Gender} & 0.6922 & \textbf{0.7058}  &  0.6811  &  0.6378  &  \textbf{0.7058}  & 0.6936   \\ 
\textbf{Hair} & 0.5792   &  \textbf{0.6061} &  0.5769  & 0.5669 &  0.5835 &  \textbf{0.6061} \\ \bottomrule
\toprule
% $\beta$ &  0.5  & 0.6 & \multicolumn{1}{c}{0.7}  & 0.8 & 0.85 & 0.9  \\ \midrule
\multirow{2}{*}{}  & \multicolumn{3}{c|}{\textbf{Clipping Value} $c$} & \multicolumn{3}{c}{\textbf{Threshold} $\beta$} \\
&  5e-4 & 1e-4 & 1e-5  & 0.8 & 0.85 & 0.9  \\ \midrule
\textbf{Gender} &  0.5753   &  0.5966 & \textbf{0.7058} & 0.6861 &  \textbf{0.7058} & 0.6381 \\ 
\textbf{Hair} &  0.3453 &  0.4099 & \textbf{0.6061}  & {0.6022}  & 0.5835 & \textbf{0.6061} \\ 
\bottomrule
\end{tabular}%

}
\end{subtable}

==> tables/tab_hyperpara_mnist.tex <==
\begin{subtable}[h]{\columnwidth}
\label{tab:projection_teachers_1}
\caption{Evaluation on MNIST and Fashion-MNIST}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\toprule
\multirow{2}{*}{}  & \multicolumn{3}{c|}{\textbf{Top-$k$}} & \multicolumn{3}{c}{\textbf{\# of Teachers}} \\ 
&  100 &  {200} & 300  & 2000  & 3000  & {4000}  \\ \midrule
\textbf{MNIST} & 0.5889  & \textbf{0.7123}  & 0.6753  & 0.5841 & 0.7061  & \textbf{0.7123}   \\ 
\textbf{Fashion} & 0.5738  & \textbf{0.6478} & 0.6088 & 0.5608 & 0.5952 & \textbf{0.6478}  \\ \bottomrule
\toprule
% $\beta$ &  0 & 0.1 & \multicolumn{1}{c}{0.3} & 0.5 & 0.7 & 0.9  \\ \midrule
\multirow{2}{*}{}  & \multicolumn{3}{c|}{\textbf{Clipping Value} $c$} & \multicolumn{3}{c}{\textbf{Threshold} $\beta$} \\
&  5e-4 & 1e-4 & 1e-5  & 0.5 & 0.7 & 0.9 \\ \midrule
\textbf{MNIST} & 0.6837 & 0.7030  & \textbf{0.7123} & 0.6921 & \textbf{0.7123} & 0.6956   \\ 
\textbf{Fashion} & 0.6054 & 0.6213 & \textbf{0.6478}  & 0.6122 & 0.6213 & \textbf{0.6478}  \\ 
\bottomrule
\end{tabular}
}
\end{subtable}

==> tables/tab_sgd.tex <==
\begin{table}[]
\centering
\caption{\small Model utility when adapting \top to DP SGD training on (a) MNIST and (b) CIFAR-10 with different privacy parameter $\eps$ and \top parameter $k$. In all cases, $\delta=10^{-5}.$ 
}\label{tab:dpsgd}


\begin{subtable}[]{\columnwidth}
	\centering
	\caption{\small MNIST}\label{tab:dpsgd-mnist}
% 	\vspace{-0.5em}
	\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|cccc}
    \toprule
        & \multicolumn{3}{c}{\small \textbf{\top}} & \multirow{2}{*}{\small \textbf{\gmdp}}  \\
    & \multicolumn{1}{c}{\small $k=0.6$}  & \multicolumn{1}{c}{\small $k=0.7$} & \multicolumn{1}{c}{\small $k=0.8$} &   \\\midrule
    $\eps=0.05$      &  73.87 {\tiny  $\pm$  4.77} &  75.81 {\tiny  $\pm$  3.59} &  77.15 {\tiny  $\pm$  2.89}           &  78.40 {\tiny  $\pm$  4.00}\\
    $\eps=0.10$     &  85.67 {\tiny  $\pm$  1.48} &  \textbf{86.12} {\tiny  $\pm$  1.39} &  85.88 {\tiny  $\pm$  1.97}    &  84.55 {\tiny  $\pm$  0.98}\\
    $\eps=0.20$     &  89.84 {\tiny  $\pm$  0.64} &  90.25 {\tiny  $\pm$  0.40} &  90.80 {\tiny  $\pm$  1.04}               &  91.17 {\tiny  $\pm$  0.37}\\
    $\eps=0.30$     &  91.21 {\tiny  $\pm$  0.53} &  91.85 {\tiny  $\pm$  0.21} &  92.35 {\tiny  $\pm$  0.53}              &  \textbf{93.31} {\tiny  $\pm$  0.42}\\
    $\eps=0.50$     &  92.83 {\tiny  $\pm$  0.52} &  93.50 {\tiny  $\pm$  0.75} &  93.82 {\tiny  $\pm$  0.46}              &  \textbf{94.38} {\tiny  $\pm$  0.24}\\
    $\eps=0.70$     &  94.41 {\tiny  $\pm$  0.19} &  94.61 {\tiny  $\pm$  0.24} &  94.65 {\tiny  $\pm$  0.27}              &  \textbf{95.08} {\tiny  $\pm$  0.10}\\
    $\eps=1.00$     &  95.13 {\tiny  $\pm$  0.33} &  95.22 {\tiny  $\pm$  0.20} &  \textbf{95.42} {\tiny  $\pm$  0.20}               &  95.41 {\tiny  $\pm$  0.26}\\
    $\eps=\infty$     &  97.94 {\tiny  $\pm$  0.19} &  98.58 {\tiny  $\pm$  0.11} &  98.79 {\tiny  $\pm$  0.09}          &  \textbf{99.08} {\tiny  $\pm$  0.04}\\
    \bottomrule
    \end{tabular}
	}
\end{subtable}


\begin{subtable}[]{\columnwidth}
	\centering
	\vspace{0.5em}
	\caption{\small CIFAR-10}\label{tab:dpsgd-cifar}
	\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|cccc}
    \toprule
    & \multicolumn{3}{c}{\small \textbf{\top}} & \multirow{2}{*}{\small \textbf{\gmdp}}  \\
			& \multicolumn{1}{c}{\small $k=0.6$}  & \multicolumn{1}{c}{\small $k=0.7$} & \multicolumn{1}{c}{\small $k=0.8$}     &   \\\midrule
 $\eps=0.025$      &  42.18 {\tiny  $\pm$  0.89} &  44.32 {\tiny  $\pm$  0.59} &  \textbf{45.87} {\tiny  $\pm$  0.97}   &  41.58 {\tiny  $\pm$  2.01}\\
 $\eps=0.050$      &  65.10 {\tiny  $\pm$  0.48} &  71.47 {\tiny  $\pm$  0.32} &  \textbf{72.03} {\tiny  $\pm$  0.25}   &  71.29 {\tiny  $\pm$  0.27}\\
 $\eps=0.075$      &  74.70 {\tiny  $\pm$  0.26} &  75.22 {\tiny  $\pm$  0.21} &  \textbf{75.62} {\tiny  $\pm$  0.15}   &  75.13 {\tiny  $\pm$  0.19}\\
 $\eps=0.10$      &  75.56 {\tiny  $\pm$  0.18} &  76.91 {\tiny  $\pm$  0.17} &  \textbf{77.65} {\tiny  $\pm$  0.20}     &  77.05 {\tiny  $\pm$  0.09}\\
 $\eps=0.20$      &  79.44 {\tiny  $\pm$  0.07} &  80.23 {\tiny  $\pm$  0.12} &  \textbf{80.76} {\tiny  $\pm$  0.08}     &  80.37 {\tiny  $\pm$  0.13}\\
 $\eps=0.30$      &  80.19 {\tiny  $\pm$  0.17} &  81.70 {\tiny  $\pm$  0.08} &  82.15 {\tiny  $\pm$  0.15}              &  \textbf{82.19} {\tiny  $\pm$  0.10}\\
 $\eps=0.40$      &  81.91 {\tiny  $\pm$  0.10} &  82.86 {\tiny  $\pm$  0.05} &  \textbf{82.82} {\tiny  $\pm$  0.13}              &  82.80 {\tiny  $\pm$  0.09}\\
 $\eps=0.60$      &  82.56 {\tiny  $\pm$  0.36} &  82.91 {\tiny  $\pm$  0.20} &  83.44 {\tiny  $\pm$  0.15}              &  \textbf{83.46} {\tiny  $\pm$  0.04}\\
 $\eps=0.80$      &  83.40 {\tiny  $\pm$  0.06} &  83.67 {\tiny  $\pm$  0.22} &  84.10 {\tiny  $\pm$  0.07}              &  \textbf{84.44} {\tiny  $\pm$  0.07}\\
 $\eps=2.00$      &  84.34 {\tiny  $\pm$  0.08} &  84.80 {\tiny  $\pm$  0.18} &  85.18 {\tiny  $\pm$  0.08}              &  \textbf{85.97} {\tiny  $\pm$  0.04}\\
 $\eps=4.00$      &  84.82 {\tiny  $\pm$  0.04} &  85.11 {\tiny  $\pm$  0.08} &  85.40 {\tiny  $\pm$  0.08}              &  \textbf{86.63} {\tiny  $\pm$  0.05}\\
 $\eps=8.00$      &  85.13 {\tiny  $\pm$  0.05} &  85.37 {\tiny  $\pm$ 0.04} & 85.62 {\tiny  $\pm$ 0.04}                  &  \textbf{87.05} {\tiny  $\pm$  0.03}\\
 $\eps=\infty$      &  85.24 {\tiny  $\pm$  0.11} &  85.46 {\tiny  $\pm$  0.12} &  85.73 {\tiny  $\pm$  0.19}          &  \textbf{87.79} {\tiny  $\pm$  0.05}\\
    \bottomrule
    \end{tabular}
	}
\end{subtable}
\vspace{-1em}
\end{table}

% \begin{table}[]
% \centering
% \caption{\small Model utility when adapting \top to DP SGD training on (a) MNIST and (b) CIFAR-10 with different privacy parameter $\eps$ and \top parameter $k$. In all cases, $\delta=10^{-5}.$ (Note that the \gmdp and )
% }\label{tab:dpsgd}


% \begin{subtable}[]{\columnwidth}
% 	\centering
% 	\caption{\small MNIST}\label{tab:dpsgd-mnist}
% % 	\vspace{-0.5em}
% 	\resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|ccccc}
%     \toprule
%         & \multicolumn{4}{c}{\small \textbf{\top}} & \multirow{2}{*}{\small \textbf{\gmdp}}  \\
% 			& \multicolumn{1}{c}{\small $k=0.6$}  & \multicolumn{1}{c}{\small $k=0.7$} & \multicolumn{1}{c}{\small $k=0.8$} & \multicolumn{1}{c}{\small $k=1.0$} &   \\\midrule
%     $\eps=0.05$      &  73.87 {\tiny  $\pm$  4.77} &  75.81 {\tiny  $\pm$  3.59} &  77.15 {\tiny  $\pm$  2.89} &  \textbf{79.79} {\tiny  $\pm$  1.96} &  78.40 {\tiny  $\pm$  4.00}\\
%     $\eps=0.10$     &  85.67 {\tiny  $\pm$  1.48} &  \textbf{86.12} {\tiny  $\pm$  1.39} &  85.88 {\tiny  $\pm$  1.97} &  85.05 {\tiny  $\pm$  1.85} &  84.55 {\tiny  $\pm$  0.98}\\
%     $\eps=0.20$     &  89.84 {\tiny  $\pm$  0.64} &  90.25 {\tiny  $\pm$  0.40} &  90.80 {\tiny  $\pm$  1.04} &  \textbf{91.48} {\tiny  $\pm$  0.50} &  91.17 {\tiny  $\pm$  0.37}\\
%     $\eps=0.30$     &  91.21 {\tiny  $\pm$  0.53} &  91.85 {\tiny  $\pm$  0.21} &  92.35 {\tiny  $\pm$  0.53} &  92.90 {\tiny  $\pm$  0.24} &  \textbf{93.31} {\tiny  $\pm$  0.42}\\
%     $\eps=0.50$     &  92.83 {\tiny  $\pm$  0.52} &  93.50 {\tiny  $\pm$  0.75} &  93.82 {\tiny  $\pm$  0.46} &  94.36 {\tiny  $\pm$  0.29} &  \textbf{94.38} {\tiny  $\pm$  0.24}\\
%     $\eps=0.70$     &  94.41 {\tiny  $\pm$  0.19} &  94.61 {\tiny  $\pm$  0.24} &  94.65 {\tiny  $\pm$  0.27} &  95.04 {\tiny  $\pm$  0.15} &  \textbf{95.08} {\tiny  $\pm$  0.10}\\
%     $\eps=1.00$     &  95.13 {\tiny  $\pm$  0.33} &  95.22 {\tiny  $\pm$  0.20} &  95.42 {\tiny  $\pm$  0.20} &  \textbf{95.66} {\tiny  $\pm$  0.22} &  95.41 {\tiny  $\pm$  0.26}\\
%     $\eps=\infty$     &  97.94 {\tiny  $\pm$  0.19} &  98.58 {\tiny  $\pm$  0.11} &  98.79 {\tiny  $\pm$  0.09} &  \textbf{99.14} {\tiny  $\pm$  0.04} &  99.08 {\tiny  $\pm$  0.04}\\
%     \bottomrule
%     \end{tabular}
% 	}
% \end{subtable}


% \begin{subtable}[]{\columnwidth}
% 	\centering
% 	\caption{\small CIFAR-10}\label{tab:dpsgd-cifar}
% % 	\vspace{-0.5em}
% 	\resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|ccccc}
%     \toprule
%     & \multicolumn{4}{c}{\small \textbf{\top}} & \multirow{2}{*}{\small \textbf{\gmdp}}  \\
% 			& \multicolumn{1}{c}{\small $k=0.6$}  & \multicolumn{1}{c}{\small $k=0.7$} & \multicolumn{1}{c}{\small $k=0.8$} & \multicolumn{1}{c}{\small $k=1.0$} &   \\\midrule
%  $\eps=0.025$      &  42.18 {\tiny  $\pm$  0.89} &  44.32 {\tiny  $\pm$  0.59} &  \textbf{45.87} {\tiny  $\pm$  0.97} &  41.36 {\tiny  $\pm$  2.14} &  41.58 {\tiny  $\pm$  2.01}\\
%  $\eps=0.050$      &  65.10 {\tiny  $\pm$  0.48} &  71.47 {\tiny  $\pm$  0.32} &  \textbf{72.03} {\tiny  $\pm$  0.25} &  71.43 {\tiny  $\pm$  0.23} &  71.29 {\tiny  $\pm$  0.27}\\
%  $\eps=0.075$      &  74.70 {\tiny  $\pm$  0.26} &  75.22 {\tiny  $\pm$  0.21} &  \textbf{75.62} {\tiny  $\pm$  0.15} &  75.01 {\tiny  $\pm$  0.28} &  75.13 {\tiny  $\pm$  0.19}\\
%  $\eps=0.10$      &  75.56 {\tiny  $\pm$  0.18} &  76.91 {\tiny  $\pm$  0.17} &  \textbf{77.65} {\tiny  $\pm$  0.20} &  77.26 {\tiny  $\pm$  0.13} &  77.05 {\tiny  $\pm$  0.09}\\
%  $\eps=0.20$      &  79.44 {\tiny  $\pm$  0.07} &  80.23 {\tiny  $\pm$  0.12} &  \textbf{80.76} {\tiny  $\pm$  0.08} &  80.38 {\tiny  $\pm$  0.10} &  80.37 {\tiny  $\pm$  0.13}\\
%  $\eps=0.30$      &  80.19 {\tiny  $\pm$  0.17} &  81.70 {\tiny  $\pm$  0.08} &  82.15 {\tiny  $\pm$  0.15} &  \textbf{82.22} {\tiny  $\pm$  0.11} &  82.19 {\tiny  $\pm$  0.10}\\
%  $\eps=0.40$      &  81.91 {\tiny  $\pm$  0.10} &  82.86 {\tiny  $\pm$  0.05} &  82.82 {\tiny  $\pm$  0.13} &  \textbf{82.88} {\tiny  $\pm$  0.04} &  82.80 {\tiny  $\pm$  0.09}\\
%  $\eps=0.60$      &  82.56 {\tiny  $\pm$  0.36} &  82.91 {\tiny  $\pm$  0.20} &  83.44 {\tiny  $\pm$  0.15} &  \textbf{83.69} {\tiny  $\pm$  0.16} &  83.46 {\tiny  $\pm$  0.04}\\
%  $\eps=0.80$      &  83.40 {\tiny  $\pm$  0.06} &  83.67 {\tiny  $\pm$  0.22} &  84.10 {\tiny  $\pm$  0.07} &  84.38 {\tiny  $\pm$  0.16} &  \textbf{84.44} {\tiny  $\pm$  0.07}\\
%  $\eps=2.00$      &  84.34 {\tiny  $\pm$  0.08} &  84.80 {\tiny  $\pm$  0.18} &  85.18 {\tiny  $\pm$  0.08} &  85.94 {\tiny  $\pm$  0.05} &  \textbf{85.97} {\tiny  $\pm$  0.04}\\
%  $\eps=4.00$      &  84.82 {\tiny  $\pm$  0.04} &  85.11 {\tiny  $\pm$  0.08} &  85.40 {\tiny  $\pm$  0.08} &  86.62 {\tiny  $\pm$  0.06} &  \textbf{86.63} {\tiny  $\pm$  0.05}\\
%  $\eps=8.00$      &  85.13 {\tiny  $\pm$  0.05} &  85.37 {\tiny  $\pm$ 0.04} & 85.62 {\tiny  $\pm$ 0.04} &  \textbf{87.06} {\tiny  $\pm$  0.04} &  87.05 {\tiny  $\pm$  0.03}\\
%  $\eps=\infty$      &  85.24 {\tiny  $\pm$  0.11} &  85.46 {\tiny  $\pm$  0.12} &  85.73 {\tiny  $\pm$  0.19} &  \textbf{87.80} {\tiny  $\pm$  0.03} &  87.79 {\tiny  $\pm$  0.05}\\
%     \bottomrule
%     \end{tabular}
% 	}
% \end{subtable}

% \end{table}
% % \sisetup{detect-weight=true,detect-inline-weight=math}
% % \begin{table}[]
% % \centering
% % \caption{\small Performance of adapting \top to DP SGD training on (a) MNIST and (b) CIFAR-10 with different privacy budgets $\eps$ and parameter $k$. We use $\delta=10^{-5}$ for all results. \fan{bold the highest numbers}
% % }\label{tab:dpsgd}
% % \begin{subtable}[]{\columnwidth}
% % 	\centering
% % 	\caption{\small MNIST}\label{tab:dpsgd-mnist}
% % % 	\vspace{-0.5em}
% % 	\resizebox{\columnwidth}{!}{%
% % 		\begin{tabular}{l|
% % 				>{\collectcell\num}R{2em}<{\endcollectcell}
% % 				@{\tiny${}\pm{}$}
% % 				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
% % 				>{\collectcell\num}R{2em}<{\endcollectcell}
% % 				@{\tiny${}\pm{}$}
% % 				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
% % 				>{\collectcell\num}R{2em}<{\endcollectcell}
% % 				@{\tiny${}\pm{}$}
% % 				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
% % 				>{\collectcell\num}R{2em}<{\endcollectcell}
% % 				@{\tiny${}\pm{}$}
% % 				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
% % 				>{\collectcell\num}R{2em}<{\endcollectcell}
% % 				@{\tiny${}\pm{}$}
% % 				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
% % 			}
% % 			\toprule
% % 			& \multicolumn{2}{c}{\small $k=0.6$}  & \multicolumn{2}{c}{\small $k=0.7$} & \multicolumn{2}{c}{\small $k=0.8$} & \multicolumn{2}{c}{\small $k=1.0$} & \multicolumn{2}{c}{\small \gmdp}  \\\midrule
% %             $\eps=0.05$ & 73.87 & 4.77 & 75.81 & 3.59 & 77.15 & 2.89 & \multicolumn{1}{c}{\textbf{79.79}} & 1.96 & 78.40 & 4.00 \\
% %             $\eps=0.10$ & 85.67 & 1.48 & 86.12 & 1.39 & 85.88 & 1.97 & 85.05 & 1.85 & 84.55 & 0.98 \\
% %             $\eps=0.20$ & 89.84 & 0.64 & 90.25 & 0.40 & 90.80 & 1.04 & 91.48 & 0.50 & 91.17 & 0.37 \\
% %             $\eps=0.30$ & 91.21 & 0.53 & 91.85 & 0.21 & 92.35 & 0.53 & 92.90 & 0.24 & 93.31 & 0.42 \\
% %             $\eps=0.50$ & 92.83 & 0.52 & 93.50 & 0.75 & 93.82 & 0.46 & 94.36 & 0.29 & 94.38 & 0.24 \\
% %             $\eps=0.70$ & 94.41 & 0.19 & 94.61 & 0.24 & 94.65 & 0.27 & 95.04 & 0.15 & 95.08 & 0.10 \\
% %             $\eps=1.00$ & 95.13 & 0.33 & 95.22 & 0.20 & 95.42 & 0.20 & 95.66 & 0.22 & 95.41 & 0.26 \\
% %             $\eps=\infty$ & 97.94 & 0.19 & 98.58 & 0.11 & 98.79 & 0.09 & 99.14 & 0.04 & 99.08 & 0.04\\				
% % 			\bottomrule
% % 		\end{tabular}%
% % 	}
% % 	\vspace{1em}
% % \end{subtable}
% % \begin{subtable}[]{\columnwidth}
% % 	\centering
% % 	\caption{\small CIFAR-10}\label{tab:dpsgd-cifar}
% % % 	\vspace{-0.5em}
% % 	\resizebox{\columnwidth}{!}{%
% % 		\begin{tabular}{l|
% % 				>{\collectcell\num}R{2em}<{\endcollectcell}
% % 				@{\tiny${}\pm{}$}
% % 				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
% % 				>{\collectcell\num}R{2em}<{\endcollectcell}
% % 				@{\tiny${}\pm{}$}
% % 				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
% % 				>{\collectcell\num}R{2em}<{\endcollectcell}
% % 				@{\tiny${}\pm{}$}
% % 				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
% % 				>{\collectcell\num}R{2em}<{\endcollectcell}
% % 				@{\tiny${}\pm{}$}
% % 				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
% % 				>{\collectcell\num}R{2em}<{\endcollectcell}
% % 				@{\tiny${}\pm{}$}
% % 				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
% % 			}
% % 			\toprule
% % 			& \multicolumn{2}{c}{\small $k=0.6$}  & \multicolumn{2}{c}{\small $k=0.7$} & \multicolumn{2}{c}{\small $k=0.8$} & \multicolumn{2}{c}{\small $k=1.0$} & \multicolumn{2}{c}{\small \gmdp}  \\\midrule
% % $\eps=0.025$  & 42.18  & 0.89 &  44.32 &  0.59 &  45.87  & 0.97 & 41.36 & 2.14 & 41.58 & 2.01 \\
% % $\eps=0.05$   & 65.10  & 0.48 &  71.47 &  0.32 &  72.03  & 0.25 & 71.43 & 0.23 & 71.29 & 0.27 \\
% % $\eps=0.075$  & 74.70  & 0.26 &  75.22 &  0.21 &  75.62  & 0.15 & 75.01 & 0.28 & 75.13 & 0.19 \\
% % $\eps=0.10$   & 75.56  & 0.18 &  76.91 &  0.17 &  77.65  & 0.20 & 77.26 & 0.13 & 77.05 & 0.09 \\
% % $\eps=0.20$   & 79.44  & 0.07 &  80.23 &  0.12 &  80.76  & 0.08 & 80.38 & 0.10 & 80.37 & 0.13 \\
% % $\eps=0.30$   & 80.19  & 0.17 &  81.70 &  0.08 &  82.15  & 0.15 & 82.22 & 0.11 & 82.19 & 0.10 \\
% % $\eps=0.40$   & 81.91  & 0.10 &  82.86 &  0.05 &  82.82  & 0.13 & 82.88 & 0.04 & 82.80 & 0.09 \\
% % $\eps=0.60$   & 82.56  & 0.36 &  82.91 &  0.20 &  83.44  & 0.15 & 83.69 & 0.16 & 83.46 & 0.04 \\
% % $\eps=0.80$   & 83.40  & 0.06 &  83.67 &  0.22 &  84.10  & 0.07 & 84.38 & 0.16 & 84.44 & 0.07 \\
% % $\eps=2.00$   & 84.34  & 0.08 &  84.80 &  0.18 &  85.18  & 0.08 & 85.94 & 0.05 & 85.97 & 0.04 \\
% % $\eps=4.00$   & 84.82  & 0.04 &  85.11 &  0.08 &  85.40  & 0.08 & 86.62 & 0.06 & 86.63 & 0.05 \\
% % $\eps=8.00$   & 85.13  & 0.05 &  85.18 &  0.12 &  85.50  & 0.08 & 87.06 & 0.04 & 87.05 & 0.03 \\
% % $\eps=\infty$ & 85.24  & 0.11 & 85.46  &  0.12 & 85.73   & 0.19 & 87.80 & 0.03 & 87.79 & 0.05  \\				
% % 			\bottomrule
% % 		\end{tabular}%
% % 	}
% % \end{subtable}

% % \end{table}


==> tables/tab_sgd_backup.tex <==
\begin{table}[]
\centering
\caption{\small Performance of \sysname when applied to SGD training on (a) MNIST and (b) CIFAR-10 with different privacy parameter $\eps$ and \top parameter $k$. In all cases, $\delta=10^{-5}.$ \fan{bold the highest numbers}
}\label{tab:dpsgd}
\begin{subtable}[]{\columnwidth}
	\centering
	\caption{\small MNIST}\label{tab:dpsgd-mnist}
% 	\vspace{-0.5em}
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{l|
				>{\collectcell\num}R{2em}<{\endcollectcell}
				@{\tiny${}\pm{}$}
				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
				>{\collectcell\num}R{2em}<{\endcollectcell}
				@{\tiny${}\pm{}$}
				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
				>{\collectcell\num}R{2em}<{\endcollectcell}
				@{\tiny${}\pm{}$}
				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
				>{\collectcell\num}R{2em}<{\endcollectcell}
				@{\tiny${}\pm{}$}
				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
				>{\collectcell\num}R{2em}<{\endcollectcell}
				@{\tiny${}\pm{}$}
				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
			}
			\toprule
			& \multicolumn{2}{c}{\small $k=0.6$}  & \multicolumn{2}{c}{\small $k=0.7$} & \multicolumn{2}{c}{\small $k=0.8$} & \multicolumn{2}{c}{\small $k=1.0$} & \multicolumn{2}{c}{\small TF-Privacy}  \\\midrule
            $\eps=0.05$ & 73.87 & 4.77 & 75.81 & 3.59 & 77.15 & 2.89 & \textbf{79.79} & 1.96 & 78.40 & 4.00 \\
            $\eps=0.10$ & 85.67 & 1.48 & \textbf{86.12} & 1.39 & 85.88 & 1.97 & 85.05 & 1.85 & 84.55 & 0.98 \\
            $\eps=0.20$ & 89.84 & 0.64 & 90.25 & 0.40 & 90.80 & 1.04 & \textbf{91.48} & 0.50 & 91.17 & 0.37 \\
            $\eps=0.30$ & 91.21 & 0.53 & 91.85 & 0.21 & 92.35 & 0.53 & 92.90 & 0.24 & \textbf{93.31} & 0.42 \\
            $\eps=0.50$ & 92.83 & 0.52 & 93.50 & 0.75 & 93.82 & 0.46 & 94.36 & 0.29 & \textbf{94.38} & 0.24 \\
            $\eps=0.70$ & 94.41 & 0.19 & 94.61 & 0.24 & 94.65 & 0.27 & 95.04 & 0.15 & \textbf{95.08} & 0.10 \\
            $\eps=1.00$ & 95.13 & 0.33 & 95.22 & 0.20 & 95.42 & 0.20 & \textbf{95.66} & 0.22 & 95.41 & 0.26 \\
            $\eps=\infty$ & 97.94 & 0.19 & 98.58 & 0.11 & 98.79 & 0.09 & \textbf{99.14} & 0.04 & 99.08 & 0.04\\				
			\bottomrule
		\end{tabular}%
	}
	\vspace{1em}
\end{subtable}
\begin{subtable}[]{\columnwidth}
	\centering
	\caption{\small CIFAR-10}\label{tab:dpsgd-cifar}
% 	\vspace{-0.5em}
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{l|
				>{\collectcell\num}R{2em}<{\endcollectcell}
				@{\tiny${}\pm{}$}
				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
				>{\collectcell\num}R{2em}<{\endcollectcell}
				@{\tiny${}\pm{}$}
				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
				>{\collectcell\num}R{2em}<{\endcollectcell}
				@{\tiny${}\pm{}$}
				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
				>{\collectcell\num}R{2em}<{\endcollectcell}
				@{\tiny${}\pm{}$}
				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
				>{\collectcell\num}R{2em}<{\endcollectcell}
				@{\tiny${}\pm{}$}
				>{\tiny\collectcell\num}R{1.2em}<{\endcollectcell}
			}
			\toprule
			& \multicolumn{2}{c}{\small $k=0.6$}  & \multicolumn{2}{c}{\small $k=0.7$} & \multicolumn{2}{c}{\small $k=0.8$} & \multicolumn{2}{c}{\small $k=1.0$} & \multicolumn{2}{c}{\small TF-Privacy}  \\\midrule
$\eps=0.025$  & 42.18  & 0.89 &  44.32 &  0.59 &  \textbf{45.87}  & 0.97 & 41.36 & 2.14 & 41.58 & 2.01 \\
$\eps=0.05$   & 65.10  & 0.48 &  71.47 &  0.32 &  \textbf{72.03}  & 0.25 & 71.43 & 0.23 & 71.29 & 0.27 \\
$\eps=0.075$  & 74.70  & 0.26 &  75.22 &  0.21 &  \textbf{75.62}  & 0.15 & 75.01 & 0.28 & 75.13 & 0.19 \\
$\eps=0.10$   & 75.56  & 0.18 &  76.91 &  0.17 &  \textbf{77.65}  & 0.20 & 77.26 & 0.13 & 77.05 & 0.09 \\
$\eps=0.20$   & 79.44  & 0.07 &  80.23 &  0.12 &  \textbf{80.76}  & 0.08 & 80.38 & 0.10 & 80.37 & 0.13 \\
$\eps=0.30$   & 80.19  & 0.17 &  81.70 &  0.08 &  82.15  & 0.15 & \textbf{82.22} & 0.11 & 82.19 & 0.10 \\
$\eps=0.40$   & 81.91  & 0.10 &  82.86 &  0.05 &  82.82  & 0.13 & \textbf{82.88} & 0.04 & 82.80 & 0.09 \\
$\eps=0.60$   & 82.56  & 0.36 &  82.91 &  0.20 &  83.44  & 0.15 & \textbf{83.69} & 0.16 & 83.46 & 0.04 \\
$\eps=0.80$   & 83.40  & 0.06 &  83.67 &  0.22 &  84.10  & 0.07 & 84.38 & 0.16 & \textbf{84.44} & 0.07 \\
$\eps=2.00$   & 84.34  & 0.08 &  84.80 &  0.18 &  85.18  & 0.08 & 85.94 & 0.05 & \textbf{85.97} & 0.04 \\
$\eps=4.00$   & 84.82  & 0.04 &  85.11 &  0.08 &  85.40  & 0.08 & 86.62 & 0.06 & \textbf{86.63} & 0.05 \\
$\eps=8.00$   & 85.13  & 0.05 &  85.18 &  0.12 &  85.50  & 0.08 & \textbf{87.06} & 0.04 & 87.05 & 0.03 \\
$\eps=\infty$ & 85.24  & 0.11 & 85.46  &  0.12 & 85.73   & 0.19 & \textbf{87.80} & 0.03 & 87.79 & 0.05  \\				
			\bottomrule
		\end{tabular}%
	}
\end{subtable}

\end{table}


